DISCERN: Identifiable Disease Evidence for Generalizable Medical Multimodal Learning

Clinical multimodal models can learn enrollment shortcuts shared across modalities and fail on new cohorts. We model these data through a latent structural causal model: disease state and background factors generate physiology through shared mechanisms, while cohorts differ in selection and measurement. Holding acquisition fixed, we identify conditional disease evidence without observing disease-state labels or recovering the full causal model. In common Gaussian coordinates, cross-cohort state alignment and natural-parameter changes identify a minimal selection statistic; conditioning on it removes enrollment-dependent evidence and yields an identifiable reference posterior within the specified shift family. State-dependent interactions can carry evidence invisible to individual-modality posteriors, motivating joint, information-preserving representations. DISCERN combines an information-lattice encoder, a latent-state model, and an outcome head through joint training. Under reversed synthetic enrollment on known latent coordinates, conditioning raises state AUROC from 0.043 to 0.883 and from 0.265 to 0.825, while random conditioning does not. Exploratory cross-database mortality experiments between eICU and MIMIC-IV improve AUROC over matched empirical risk minimization by 0.036 and 0.035. Learned-coordinate diagnostics distinguish preservation of state information from identification of the coordinates required by the estimator.

==> archive/A_examples.tex <==
\section{Exact examples of enrollment shortcuts and joint evidence}
\label{app:examples}

These examples give exact population errors for specified mechanisms (Figure~\ref{fig:examples}). They illustrate Sections~\ref{sec:setting} and~\ref{sec:theory}; they are not fitted \method{} or ERM performance.

\begin{figure}[H]
\centering
\includegraphics[width=.9\linewidth]{figures/fig_examples.pdf}
\caption{\textbf{Analytical illustrations.} (a)~An enrollment reversal changes the error of a background-only rule from $0.1$ to $0.9$, while a rule that uses the specified mechanism through the residual has error $0.02275$ in both cohorts. (b)~Contours at Mahalanobis radii one and two for two Gaussian states with correlations $+0.8$ and $-0.8$. Each single-view posterior is uninformative, whereas the joint interaction yields error $0.20483$. Contours are analytical densities; no error bars apply.}
\label{fig:examples}
\end{figure}

\paragraph{Enrollment-induced shortcut.}
This is the selection of Figure~\ref{fig:motivation}a with one background factor. Let population signs $S,B\in\{-1,+1\}$ be independent and balanced, and let the inclusion indicator $R$ satisfy
\begin{equation}
P(R=1\mid S,B,e)=\begin{cases}a_e,& B=S,\\ 1-a_e,& B\neq S.\end{cases}
\label{eq:inclusion}
\end{equation}
Then $P(R=1)=1/2$, $P(S=+1\mid R=1,e)=1/2$ and $P(B=S\mid R=1,e)=a_e$. The rule $h_B=B$ has selected-cohort error $1-a_e$: $0.1$ for the source law $a_e=0.9$ and $0.9$ for the target law $a_e=0.1$. Let $D=S+B+\epsilon$ with $\epsilon\sim\mathcal N(0,0.5^2)$ independent of $(S,B)$ and of the inclusion noise, inclusion depending only on $(S,B,e)$. With the parents and the mechanism known,
\begin{equation}
h_{\mathrm{mech}}=\operatorname{sign}(D-B),\qquad P(h_{\mathrm{mech}}\neq S\mid R=1,e)=\Phi(-2)\simeq0.02275.
\end{equation}
Conditioning on $B$ preserves the disease mechanism while removing the selected-cohort association from its evidence, as in the conditional sub-model evidence of Appendix~\ref{app:proofs}. The mechanism and parents are given here; this discrete example lies outside the Gaussian alignment theorem, and target selection can itself carry useful evidence, which is the price in Equation~\eqref{eq:gap}.

\paragraph{Interaction invisible to separate posteriors.}
In a separate two-view model take balanced $S$, independent standard Gaussian noises $\epsilon_1,\epsilon_2$, and
\begin{equation}
X_1=D_1=\epsilon_1,\qquad X_2=D_2=\rho S D_1+\sqrt{1-\rho^2}\,\epsilon_2,\qquad \rho=0.8.
\end{equation}
Both single-view state-conditionals are standard normal, so each single-view Bayes posterior equals $1/2$, and any rule that uses only those two posterior values has error $1/2$. In contrast,
\begin{equation}
\log\frac{p(x_1,x_2\mid S=+1)}{p(x_1,x_2\mid S=-1)}=\frac{2\rho x_1x_2}{1-\rho^2},\qquad R^*_{\mathrm{joint}}=\frac{\arccos\rho}{\pi}\simeq0.20483.
\end{equation}
The Bayes rule is $\operatorname{sign}(X_1X_2)$. The loss concerns separate-posterior compression, not all late fusion; in Figure~\ref{fig:motivation}a the laboratory modality $X^{(2)}$ observes both $D_1$ and $D_2$, so this particular bottleneck does not apply there.


==> archive/F_related.tex <==
\section{Related work}
\label{app:related}

\paragraph{Medical multimodal learning.}
Fusion architectures for imaging and electronic health records span early, late and hybrid designs~\citep{huang2020fusion,acosta2022multimodal,kline2022multimodal}; MedFuse handles paired and unpaired time series and radiographs~\citep{hayat2022medfuse}, HAIM combines tabular, temporal, text and image embeddings~\citep{soenksen2022integrated}, and contrastive objectives pre-train imaging encoders from clinical tables~\citep{hager2023best}. Missing-modality transformers~\citep{ma2022multimodal,zhang2022m3care} and modality-balancing objectives~\citep{wang2020what,peng2022balanced} address in-distribution failure modes; surveys organize the space~\citep{stahlschmidt2022multimodal,baltrusaitis2019multimodal,liang2024foundations}. Recent work disentangles shared from modality-specific diagnostic information in paired ECG and cardiac MRI~\citep{tonekaboni2025representation}, treats modality missingness as informative through a latent health state, with experiments on MIMIC-IV and eICU~\citep{liang2025causal}, and benchmarks EHR and chest X-ray fusion within one health system~\citep{elsharief2025medmod}. These works assume representative training cohorts and evaluate on held-out patients of the same cohort or health system. Shortcut learning in medical imaging~\citep{zech2018variable,degrave2021ai,winkler2019association,oakdenrayner2020hidden,geirhos2020shortcut,brown2023detecting} and deployment failures~\citep{wong2021external,nestor2019feature,finlayson2021clinician} document the cost. \citet{huang2021what} explain when multiple modalities provably outperform a single one by the quality of a shared latent representation; \citet{lu2023theory} give a learning-theoretic account based on heterogeneity between modalities and a learnable connection between them. More recent analyses show that contrastive alignment captures mainly redundant information and can miss unique and synergistic terms~\citep{dufumier2025what}, that whether alignment helps depends on the balance of redundant and unique information~\citep{tjandrasuwita2025understanding}, and that modality competition can be rebalanced by a game-theoretic regularizer~\citep{kontras2025balancing}. These address in-distribution learning; none models how a disease generates the modalities or how their evidence changes across cohorts.

\paragraph{Robust machine learning.}
IRM~\citep{arjovsky2019invariant}, V-REx~\citep{krueger2021out}, GroupDRO~\citep{sagawa2020distributionally}, CORAL~\citep{sun2016deep}, LISA~\citep{yao2022improving}, JTT~\citep{liu2021just}, DFR~\citep{kirichenko2023last}, SWAD~\citep{cha2021swad} and test-time adaptation~\citep{iwasawa2021test,wang2021tent} form the standard baselines; DomainBed~\citep{gulrajani2021search} and WILDS~\citep{koh2021wilds} show how hard ERM is to beat, and \citet{rosenfeld2021risks,kamath2021does} show when invariance criteria fail. NuRD~\citep{puli2022nuisance} and invariant-feature subspace recovery~\citep{wang2022provable} are the closest statistical targets; anchor regression~\citep{rothenhausler2021anchor}, invariant causal prediction~\citep{peters2016causal,rojascarulla2018invariant} and conditional variance penalties~\citep{heinzedeml2021conditional} condition on observed labels or anchors. Clinical DG frameworks~\citep{zhang2021empirical} and harmonization~\citep{johnson2007adjusting,fortin2018harmonization} address site effects; \citet{subbaswamy2019preventing,subbaswamy2020development,castro2020causality} argue for causal modelling of clinical shifts. In critical care, multi-database studies find that internal validation overestimates external performance and that site-specific features act as shortcuts for mortality prediction~\citep{allyn2026multisource}, that sepsis models degrade across MIMIC-IV, eICU and HiRID with the best adaptation strategy depending on target data~\citep{tranchellini2026evaluating}, and that anchor regression with the database as anchor aids transfer across nine ICU databases~\citep{londschien2026domain}. Causal representation learning builds on identifiability results for finite Gaussian mixtures~\citep{yakowitz1968identifiability}, nonlinear ICA with auxiliary variables~\citep{hyvarinen2016unsupervised,hyvarinen2019nonlinear,khemakhem2020variational}, mixture priors with piecewise-affine decoders~\citep{kivva2022identifiability}, content and style from augmentations~\citep{vonkugelgen2021self,zimmermann2021contrastive,daunhawer2023identifiability}, multi-view partial observability~\citep{yao2024multiview,sturma2023unpaired}, sparse cross-modal causal structure in biomedical observations~\citep{sun2025causal}, partial disentanglement for adaptation~\citep{kong2022partial} and sparsity~\citep{lachapelle2022disentanglement}, is unified by viewing identification as preserving known invariances~\citep{yao2025unifying}, and is limited by the impossibility of unsupervised disentanglement without inductive bias~\citep{locatello2019challenging}. Latent structure can remain identifiable under selection bias in linear Gaussian models~\citep{dai2025latent}, a setting close to our enrollment shift but aimed at causal discovery rather than transfer. Our result concerns a function of the latent vector, the evidence about an unobserved state that survives enrollment changes, and its alignment and coordinate premises are explicit.


==> figures/archive/fig1a_generative.tex <==
% Figure 1(a): the generative view of multimodal clinical data (illustrated layout).
% Coordinates are in units of 1/100 of a 1254-px design canvas, y pointing down.
% Teal: disease state and its mechanisms; sand: background B; light blue: physiology D;
% coloured arrows: which latent coordinates each modality observes; orange dashed: what a cohort changes.
% Icons (figures/icon_*.png) are cropped from the authors' illustration with a transparent background.
\definecolor{fS}{RGB}{0,138,118}%
\definecolor{fSfill}{RGB}{204,240,232}%
\definecolor{fD}{RGB}{30,110,225}%
\definecolor{fDfill}{RGB}{222,236,253}%
\definecolor{fB}{RGB}{150,120,70}%
\definecolor{fBfill}{RGB}{243,234,214}%
\definecolor{fimg}{RGB}{20,112,235}%
\definecolor{fimgbg}{RGB}{228,243,254}%
\definecolor{flab}{RGB}{240,160,20}%
\definecolor{flabbg}{RGB}{254,246,231}%
\definecolor{fphy}{RGB}{228,72,72}%
\definecolor{fphybg}{RGB}{254,230,230}%
\definecolor{fend}{RGB}{140,45,210}%
\definecolor{fendbg}{RGB}{239,233,254}%
\definecolor{fscm}{RGB}{226,249,243}%
\definecolor{fcoh}{RGB}{217,114,42}%
\begin{tikzpicture}[x=0.72cm,y=-0.72cm,
  font=\footnotesize,
  lat/.style={circle,minimum size=5.6mm,inner sep=0pt,line width=.8pt},
  D/.style={lat,draw=fD,fill=fDfill},
  B/.style={lat,draw=fB,fill=fBfill},
  S/.style={circle,minimum size=7.2mm,inner sep=0pt,line width=1.3pt,draw=fS,fill=fSfill},
  X/.style={circle,minimum size=6.6mm,inner sep=0pt,line width=1pt,fill=white},
  mech/.style={-{Stealth[length=1.6mm]},draw=fS,line width=.8pt},
  obs/.style={-{Stealth[length=1.5mm]},line width=.75pt},
  noise/.style={-{Stealth[length=1.3mm]},draw=gray!80,line width=.6pt},
  coh/.style={-{Stealth[length=1.4mm]},draw=fcoh,dashed,line width=.7pt},
  cohtag/.style={fcoh,font=\scriptsize,inner sep=1pt},
  title/.style={font=\footnotesize\bfseries,align=center},
]
\useasboundingbox (0.15,0.5) rectangle (12.45,12.8);
% ---------------- modality regions
\fill[fimgbg,rounded corners=14pt] (0.2,0.55) rectangle (4.85,3.9);
\fill[flabbg,rounded corners=14pt] (7.65,0.55) rectangle (12.4,3.95);
\fill[fphybg,rounded corners=14pt] (0.2,8.45) rectangle (5.2,11.5);
\fill[fendbg,rounded corners=14pt] (7.5,8.1) rectangle (12.4,11.6);
% ---------------- latent SCM
\draw[fS!70,dashed,line width=.6pt,fill=fscm] (6.25,5.85) ellipse (3.75 and 2.9);
\node[font=\footnotesize\bfseries,fS!70!black] at (6.25,1.95) {Latent SCM};
\node[font=\scriptsize,fS!60!black,align=center] at (6.25,2.5) {shared by\\[-2pt]all cohorts};
% ---------------- icons
\node at (3.3,1.85) {\includegraphics[width=1.9cm]{figures/icon_brain.png}};
\node at (11.25,2.05) {\includegraphics[width=1.35cm]{figures/icon_tubes.png}};
\node at (4.4,9.95) {\includegraphics[width=0.7cm]{figures/icon_heart.png}};
\node at (11.25,9.55) {\includegraphics[width=1.0cm]{figures/icon_clip.png}};
% ECG trace
\draw[fphy,line width=.6pt] (0.55,10.15) -- (1.0,10.15) -- (1.12,9.85) -- (1.22,10.55) -- (1.34,9.6) -- (1.46,10.3) -- (1.56,10.15)
  -- (2.0,10.15) -- (2.12,9.85) -- (2.22,10.55) -- (2.34,9.6) -- (2.46,10.3) -- (2.56,10.15)
  -- (3.0,10.15) -- (3.12,9.85) -- (3.22,10.55) -- (3.34,9.6) -- (3.46,10.3) -- (3.56,10.15) -- (3.85,10.15);
% ---------------- latent nodes
\node[S] (S) at (6.25,4.9) {$S$};
\node[B] (B1) at (4.2,5.2) {$B_1$};
\node[B] (B2) at (8.5,5.2) {$B_2$};
\node[D] (D1) at (4.62,6.65) {$D_1$};
\node[D] (D2) at (6.25,7.8) {$D_2$};
\node[D] (D3) at (7.9,6.65) {$D_3$};
% ---------------- modality and endpoint nodes
\node[X,draw=fimg] (X1) at (1.2,2.3) {$X^{(1)}$};
\node[title] at (1.2,3.3) {Imaging};
\node[X,draw=flab] (X2) at (9.25,2.05) {$X^{(2)}$};
\node[title] at (11.0,3.4) {Laboratory};
\node[X,draw=fphy] (X3) at (2.2,9.35) {$X^{(3)}$};
\node[title] at (2.45,11.0) {Physiological signals};
\node[X,draw=fend] (Y) at (9.65,9.45) {$Y$};
\node[title] at (9.65,10.65) {Clinical endpoint};
\node[font=\scriptsize] at (9.65,11.15) {diagnosis / prognosis};
% ---------------- mechanisms (fixed across cohorts)
\draw[mech] (S) -- (D1);
\draw[mech] (S) -- (D2);
\draw[mech] (S) -- (D3);
\draw[mech] (B1) -- (D1);
\draw[mech] (D1) -- (D2);
\draw[mech] (B2) -- (D3);
% ---------------- observation maps
\draw[obs,draw=fimg] (B1) to[out=160,in=-40] (X1);
\draw[obs,draw=fimg] (D1) to[out=175,in=-70] (X1);
\draw[obs,draw=flab] (D1) to[out=20,in=-110] (X2);
\draw[obs,draw=flab] (B2) to[out=95,in=-60] (X2);
\draw[obs,draw=flab] (D2) to[out=5,in=-50] (X2);
\draw[obs,draw=fphy] (D2) to[out=190,in=20] (X3);
\draw[obs,draw=fphy] (D3) to[out=235,in=15] (X3);
\draw[obs,draw=fend] (D3) to[out=-40,in=150] (Y);
\draw[obs,draw=fend] (B2) to[out=-30,in=75] (Y);
% ---------------- private variation
\node[gray!60!black,font=\scriptsize] (V1) at (0.55,1.05) {$\xi_1$};
\draw[noise] (V1) to[bend left=25] (X1.north west);
\node[gray!60!black,font=\scriptsize] (V2) at (8.1,1.05) {$\xi_2$};
\draw[noise] (V2) to[bend left=25] (X2.north west);
\node[gray!60!black,font=\scriptsize] (V3) at (0.75,8.8) {$\xi_3$};
\draw[noise] (V3) to[bend left=25] (X3.west);
% ---------------- what a cohort changes (orange dashed)
\node[cohtag,anchor=south] (prev) at (6.25,3.65) {selection $p_e(s,b)$};
\draw[coh] (prev) -- (S);
\draw[coh,{Stealth[length=1.4mm]}-{Stealth[length=1.4mm]}] (B1) to[bend left=35] (S);
\draw[coh,{Stealth[length=1.4mm]}-{Stealth[length=1.4mm]}] (S) to[bend left=35] (B2);
\node[cohtag] (c1) at (2.3,0.95) {$c_1(e)$};
\draw[coh] (c1) to[bend right=20] (X1.north east);
\node[cohtag] (c2) at (10.45,0.9) {$c_2(e)$};
\draw[coh] (c2) to[bend left=20] (X2.north east);
\node[cohtag] (c3) at (3.2,8.72) {$c_3(e)$};
\draw[coh] (c3) to[bend right=25] (X3.north east);
\node[cohtag] (lp) at (8.35,9.45) {$c_Y(e)$};
\draw[coh] (lp) -- (Y.west);
% ---------------- legend
\draw[gray!50,rounded corners=3pt,fill=white] (0.2,11.9) rectangle (12.4,12.75);
\node[S,minimum size=3.2mm,line width=.9pt] at (0.55,12.33) {};
\node[anchor=west,font=\scriptsize] at (0.78,12.33) {disease state $S$};
\node[B,minimum size=3.2mm] at (3.6,12.33) {};
\node[anchor=west,font=\scriptsize] at (3.83,12.33) {background $B$};
\node[D,minimum size=3.2mm] at (6.6,12.33) {};
\node[anchor=west,font=\scriptsize] at (6.83,12.33) {physiology $D$};
\draw[coh] (9.4,12.33) -- (9.95,12.33);
\node[anchor=west,font=\scriptsize] at (10.0,12.33) {cohort-specific};
\end{tikzpicture}


==> figures/fig2_method.tex <==
% Figure 2: the DISCERN pipeline (views -> lattice -> aligned state model -> selection statistic -> conditional evidence -> outcome head)
\definecolor{cdis}{HTML}{1f8a70}%
\definecolor{ccoh}{HTML}{d9722a}%
\definecolor{cview}{HTML}{2a6fbd}%
\definecolor{cgray}{HTML}{6b6a66}%
\definecolor{cvio}{HTML}{4a3aa7}%
\begin{tikzpicture}[
  font=\footnotesize,
  box/.style={rectangle,rounded corners=2pt,draw=cgray,line width=.5pt,fill=white,align=center,inner sep=3.5pt},
  mod/.style={box,draw=cview,fill=cview!8,minimum width=10mm,minimum height=5.5mm},
  stage/.style={box,draw=cgray!70,fill=cgray!4,text width=30mm,minimum height=17mm},
  ann/.style={cgray,font=\scriptsize,align=center},
  arr/.style={-{Stealth[length=1.8mm]},draw=cgray,line width=.7pt},
  darr/.style={-{Stealth[length=1.8mm]},draw=ccoh,line width=.7pt,dashed},
]
\node[mod] (x2) at (0,0) {$X^{(2)}$};
\node[mod] (x1) at (0,0.85) {$X^{(1)}$};
\node[mod] (x3) at (0,-0.85) {$X^{(3)}$};
\node[stage,text width=33mm,minimum height=22mm] (enc) at (2.9,0) {\textbf{information lattice}\\[2pt]
  {\scriptsize\setlength{\fboxsep}{1.8pt}
  \colorbox{cdis!25}{\strut shared $\{1,2,3\}$}\\[1.5pt]
  \colorbox{cview!15}{\strut $\{1,2\}$}\;\colorbox{cview!15}{\strut $\{1,3\}$}\;\colorbox{cview!15}{\strut $\{2,3\}$}\\[1.5pt]
  \colorbox{cgray!12}{\strut $\{1\}$}\;\colorbox{cgray!12}{\strut $\{2\}$}\;\colorbox{cgray!12}{\strut $\{3\}$}}\\[2pt]
  align $+$ reconstruct\\ no labels; $\hat z$\; {\color{cgray}\scriptsize Prop.~\ref{prop:lattice}}};
\draw[arr] (x1.east) -- (enc.west |- x1); \draw[arr] (x2.east) -- (enc.west |- x2); \draw[arr] (x3.east) -- (enc.west |- x3);
\node[stage] (em) at (6.55,0.95) {\textbf{aligned state model}\\ $\hat z\mid s,e\sim\mathcal N(\mu_{es},\Sigma_s)$\\ EM on source cohorts,\\ aligned by Prop.~\ref{prop:align}};
\node[stage] (sel) at (10.2,0.95) {\textbf{selection statistic}\\ $\Sigma_s^{-1}(\mu_{es}-\bar\mu_s)\ \to$ SVD\\ $U=\Bb^\top\hat z$\\ {\color{cgray}\scriptsize Thm.~\ref{thm:evidence}}};
\node[stage,fill=cdis!6,draw=cdis!70] (ev) at (10.2,-1.05) {\textbf{conditional evidence}\\ $\hat T_s=\hat\ell_s(\hat z)-\hat\ell_s(\Bb^\top\hat z)$\\ $\hat q(s\mid\hat z)\propto\pi_s e^{\hat T_s}$\\ {\color{cgray}\scriptsize joint minus marginal}};
\node[stage,fill=ccoh!6,draw=ccoh!80,text width=27mm] (head) at (13.6,-0.05) {\textbf{outcome head}\\ $h_\theta\big(r(X),\log\hat q_s/\hat q_0\big)$\\ continuous path $r$\\ {\color{cgray}\scriptsize Prop.~\ref{prop:decomp}}};
\node[ann] (r) at (6.55,-1.05) {continuous features $r(X)$\\ (lattice coordinates)};
\draw[arr] (enc.east |- em.west) -- (em.west);
\draw[arr] (em) -- (sel);
\draw[arr] (sel) -- (ev);
\draw[arr] (em.south east) -- (ev.north west);
\draw[arr] (ev.east) -- (head.west |- ev.east);
\draw[arr] (enc.east |- r.west) -- (r.west);
\draw[arr] (r.east) -- (head.west |- r.east);
\node[ann,anchor=north] at (7.6,-2.05) {source fitting: lattice, state model, selection basis and head; frozen before deployment; target cohorts supply unlabeled observations only};
\end{tikzpicture}

